CoRelation: Boosting Automatic ICD Coding Through Contextualized Code Relation Learning

Automatic International Classification of Diseases (ICD) coding plays a crucial role in the extraction of relevant information from clinical notes for proper recording and billing. One of the most important directions for boosting the performance of automatic ICD coding is modeling ICD code relations. However, current methods insufficiently model the intricate relationships among ICD codes and often overlook the importance of context in clinical notes. In this paper, we propose a novel approach, a contextualized and flexible framework, to enhance the learning of ICD code representations. Our approach, unlike existing methods, employs a dependent learning paradigm that considers the context of clinical notes in modeling all possible code relations. We evaluate our approach on six public ICD coding datasets and the experimental results demonstrate the effectiveness of our approach compared to state-of-the-art baselines.

==> files/experiment.tex <==
\section{Experiments}

\subsection{Experiment Settings}
In this section, we introduce the experimental settings, which include the datasets, baselines, and evaluation metrics. \emph{Due to space limitations, we have included the \textbf{implementation details} of our model in the Appendix of the supplementary file.}


% \subsubsection{Datasets} 
% To evaluate our method, we utilize the ICD coding datasets derived from the MIMIC-III~\cite{johnson2016mimic} and MIMIC-IV~\cite{johnson2020mimic} projects. Specifically, we follow the settings of~\cite{mullenbach2018explainable, yuan2022code} to create the MIMIC-III-50 and MIMIC-III-Full datasets, and the settings of~\cite{nguyen2023mimic} to create the MIMIC-IV-ICD9-50, MIMIC-IV-ICD9-Full, MIMIC-IV-ICD10-50, and MIMIC-IV-ICD10-Full datasets. The statistics of the six datasets are presented in Table~\ref{table:datasets}. For the MIMIC-III dataset, we divide it into two settings based on the number of ICD codes: the \textbf{50} setting focuses on evaluating the top 50 most frequent ICD codes, and the \textbf{Full} setting focuses on evaluating all potential ICD codes. For the MIMIC-IV dataset, we divide it into four settings based on the ICD code version\footnote{\url{https://www.cdc.gov/nchs/icd/icd9cm.htm,https://www.cdc.gov/nchs/icd/icd10cm.htm}} and the number of codes.

\subsubsection{Datasets} 
To evaluate our method, we utilize the ICD coding datasets derived from the MIMIC-III~\cite{johnson2016mimic} and MIMIC-IV~\cite{johnson2020mimic} projects. Specifically, we follow the settings of~\cite{mullenbach2018explainable, yuan2022code} to create the MIMIC-III-50 and MIMIC-III-Full datasets, and the settings of~\cite{nguyen2023mimic} to create the MIMIC-IV-ICD9-50, MIMIC-IV-ICD9-Full, MIMIC-IV-ICD10-50, and MIMIC-IV-ICD10-Full datasets. The \textbf{50} setting focuses on evaluating the top 50 most frequent ICD codes, and the \textbf{Full} setting focuses on evaluating all potential ICD codes. 
The statistics of the six datasets are presented in Table~\ref{table:datasets}.

\begin{table}[t]
\centering
\caption{Statistics of the six datasets.}
\label{table:datasets}
\resizebox{0.49\textwidth}{!}{
\tabcolsep=0.05cm
\begin{tabular}{l|cc|cc|cc}
\hline
Database & \multicolumn{2}{c|}{{\textbf{MIMIC-III}}} & \multicolumn{4}{c}{\textbf{MIMIC-IV}}                         \\  \hline
Code Version& \multicolumn{2}{c|}{{ICD9}}                           & \multicolumn{2}{c|}{{ICD9}} & \multicolumn{2}{c}{{ICD10}} \\ \hline
Settings & 50                     & Full                   & 50          & Full       & 50          & Full        \\ \cline{1-7} 
                  % code ver.   & ICD9                  & ICD9                  & ICD9       & ICD9      & ICD10      & ICD10      \\
\# of codes in $\mathcal{C}$       & 50                     & 8,922                  & 50          & 11,331     & 50          & 26,096      \\
Training size  & 8,066                  & 47,723                 & 170,664     & 180,553    & 104,077     & 110,442     \\
Validation size    & 1,573                  & 1,631                  & 6,406       & 7,110      & 3,805       & 4,017       \\
Testing  size & 1,729                  & 3,372                  & 12,405      & 13,709     & 7,368       & 7,851       \\ 
Avg \# of tokens   & 1,478                  & 1,434                  & 1,499      & 1,459     &  1,687       &  1,662       \\ \hline
\end{tabular}
}

\end{table}



% \subsubsection{Baselines}
% For baseline selection, we primarily consider those representative works that utilize only the discharge notes or additional ICD code knowledge.
% Works~\cite{liu2022treeman, ng2023modelling, yang2022multi,niu2023retrieve,zhang2022automatic} require additional annotation data, information source, or multiple retrieval stages are not considered for fairness.
% In detail, we select the following works as baselines and divide them into two classes based on whether they utilize pre-trained language models (PLM) as encoders. \emph{The reported results are obtained from the \textbf{provided trained models} or \textbf{the original papers} if the codes are not available. The baseline results of MIMIC-IV settings are collected from~\cite{nguyen2023mimic}.} 

% Non-PLM methods, including CAML~\cite{mullenbach2018explainable}, MultiResCNN~\cite{li2020icd}, HyperCore~\cite{cao2020hypercore}, LAAT and JointLAAT~\cite{vu2021label}, MSMN~\cite{yuan2022code}, TwoStage~\cite{nguyen2023two}.
% PLM methods, including \textit{KEPT}\footnote{For \textit{KEPT} we only report the 50 setting, since the reported Full setting results utilize multiple methods to perform a multi-stage retrieval.}~\cite{yang2022knowledge}, \textit{HiLAT}~\cite{liu2022hierarchical}, \textit{PLM-ICD}~\cite{huang-etal-2022-plm}. 

\subsubsection{Baselines}
We divide baselines into two classes based on whether they utilize pre-trained language models (PLMs) as encoders:
(1) \textbf{Non-PLM} methods include CAML~\cite{mullenbach2018explainable}, MultiResCNN~\cite{li2020icd}, HyperCore~\cite{cao2020hypercore}, LAAT and JointLAAT~\cite{vu2021label}, MSMN~\cite{yuan2022code}, and TwoStage~\cite{nguyen2023two}; and (2)
\textbf{PLM} methods include {KEPT}\footnote{For {KEPT}, we only report the results of the 50 setting since the Full setting results utilize multiple methods to perform a multi-stage retrieval.}~\cite{yang2022knowledge}, {HiLAT}~\cite{liu2022hierarchical}, and {PLM-ICD}~\cite{huang-etal-2022-plm}. 

We obtain the results of baselines either from the released trained models or the original papers if the codes are unavailable. It is worth noting that these models~\cite{liu2022treeman, ng2023modelling, yang2022multi,niu2023retrieve,zhang2022automatic} are not listed in baselines since they require additional information, such as annotation data, information source, and multiple retrieval stages.


% \subsubsection{Evaluation Metrics}
% We adhere to conventional settings established by previous studies~\cite{mullenbach2018explainable, vu2021label, yuan2022code}, reporting Macro Micro AUC, Macro Micro F1, and P@5 metrics for the three \textbf{50} settings. For the three \textbf{Full} settings, we report Macro Micro AUC, Macro Micro F1, and P@8 metrics. To enable a thorough comparison with recent state-of-the-art (SOTA) works, we additionally include the P@8 metric for MIMIC-III-50 and the P@5, P@15 metrics for the MIMIC-III-Full.

\subsubsection{Evaluation Metrics}
Following previous studies~\cite{mullenbach2018explainable, vu2021label, yuan2022code}, we report Macro \& Micro AUC, Macro \& Micro F1, and Precision at K (P@$\mathcal{K}$) metrics, where $\mathcal{K}=5,8, 15$ for different settings. The \textbf{Bold} notation indicates the best results among non-PLM techniques, while \underline{Underline} notation signifies the best results when considering the PLM setting. %\textcolor{red}{Furthermore, due to the small size and instability of the MIMIC-III-50 setting, we report the average results over five rounds for the MIMIC-III-50.}
% for the \textbf{50} settings. For the \textbf{Full} settings, we report Macro Micro AUC, Macro Micro F1, and P@8 metrics. To enable a thorough comparison with recent state-of-the-art (SOTA) works, we additionally include the P@8 metric for MIMIC-III-50 and the P@5, P@15 metrics for the MIMIC-III-Full.


% \begin{table}[h]
% \footnotesize
% \centering
% \tabcolsep=0.11cm
% \begin{tabular}{lcccccc}
% \hline
% \multicolumn{7}{c}{\textbf{MIMIC-III-50}}                                                                                 \\
% \multicolumn{1}{c}{Method} & \multicolumn{2}{c}{AUC}       & \multicolumn{2}{c}{F1}        & \multicolumn{2}{c}{Pre}       \\ \hline
% \textbf{Non-PLM}          & Macro         & Micro         & Macro         & Micro         & P@5           & P@8           \\ \hline
% CAML                      & 87.5          & 90.9          & 53.2          & 61.4          & 60.9          & -             \\
% MultiResCNN               & 89.9          & 92.8          & 60.6          & 67.0          & 64.1          & -             \\
% HyperCore                 & 89.5          & 92.9          & 60.9          & 66.3          & 63.2          & -             \\
% LAAT                      & 92.5          & 94.6          & 66.6          & 71.5          & 67.5          & 54.7          \\
% JointLAAT                 & 92.5          & 94.6          & 66.1          & 71.6          & 67.1          & 54.6          \\
% TwoStage                  & 92.6          & 94.5          & 68.9          & 71.8          & 66.7          & -             \\
% MSMN                      & 92.8          & 94.7          & 68.3          & 72.5          & 68.0          & 54.8          \\
% \textbf{CoRelation}                & \textbf{93.3} & \textbf{95.1} & \textbf{69.3} & \textbf{73.1} & \textbf{68.3} & \textbf{55.6} \\ \hline
% \textbf{PLM}              &               &               &               &               &               &               \\ \hline
% \textit{HiLAT}                     & 92.7          & 95.0          & 69.0          & {\underline{73.5}}    & 68.1          & 55.4          \\
% \textit{PLM-ICD}                   & 90.2          & 92.7          & 64.8          & 69.6          & 65.0          & 53.0          \\
% \textit{KEPT}                      & 92.6          & 94.8          & 68.9          & 72.9          & 67.3          & 54.8          \\ \hline
% \end{tabular}
% \caption{Results on the MIMIC-III-50 test set.}
% \label{table:MIMIC-50}
% \end{table}

\begin{table}[t]
\centering
\caption{Results on the MIMIC-III-50 test set.}
\label{table:MIMIC-50}
% \tabcolsep=0.11cm
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l|l|cccccc}
\hline
\multirow{2}{*}{Category}&\multirow{2}{*}{Method} & \multicolumn{2}{c}{AUC}       & \multicolumn{2}{c}{F1}        & \multicolumn{2}{c}{Pre}       \\ \cline{3-8}
     &    & Macro         & Micro         & Macro         & Micro         & P@5           & P@8           \\ \hline
\multirow{3}{*}{{PLM}}
&{HiLAT}                     & 92.7          & 95.0          & 69.0          & {\underline{73.5}}    & 68.1          & 55.4          \\
&{PLM-ICD}                   & 90.2          & 92.7          & 64.8          & 69.6          & 65.0          & 53.0          \\
&{KEPT}                      & 92.6          & 94.8          & 68.9          & 72.9          & 67.3          & 54.8          \\ \hline

\multirow{8}{*}{\makecell[l]{Non-PLM}} 
&CAML                      & 87.5          & 90.9          & 53.2          & 61.4          & 60.9          & -             \\
&MultiResCNN               & 89.9          & 92.8          & 60.6          & 67.0          & 64.1          & -             \\
&HyperCore                 & 89.5          & 92.9          & 60.9          & 66.3          & 63.2          & -             \\
&LAAT                      & 92.5          & 94.6          & 66.6          & 71.5          & 67.5          & 54.7          \\
&JointLAAT                 & 92.5          & 94.6          & 66.1          & 71.6          & 67.1          & 54.6          \\
&TwoStage                  & 92.6          & 94.5          & 68.9          & 71.8          & 66.7          & -             \\
&MSMN                      & 92.8          & 94.7          & 68.3          & 72.5          & 68.0          & 54.8          \\

&\cellcolor{blue!25}{\model}                & \cellcolor{blue!25}\textbf{93.3} & \cellcolor{blue!25}\textbf{95.1} & \cellcolor{blue!25}\textbf{69.3} & \cellcolor{blue!25}\textbf{73.1} & \cellcolor{blue!25}\textbf{68.3} & \cellcolor{blue!25}\textbf{55.6} \\ \hline

\end{tabular}
}

\end{table}



% \begin{table}[h]
% \footnotesize
% \centering
% \tabcolsep=0.21cm
% \begin{tabular}{lccccc}
% \hline
% \multicolumn{6}{c}{\textbf{MIMIC-IV-ICD9-50}}                                                                                                                                                                                  \\
% \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{AUC}                                               & \multicolumn{2}{c}{F1}                                                & Pre                               \\ \cline{2-6} 
% \multicolumn{1}{c}{}                       & Macro                             & Micro                             & Macro                             & Micro                             & P@5                               \\ \hline
% CAML                                       & 93.1                              & 94.1                              & 65.3                              & 69.2                              & 58.6                              \\
% LAAT                                       & 94.9                              & 96.3                              & 70.0                              & 74.5                              & 62.0                              \\
% JointLAAT                                  & 94.9                              & 96.3                              & 69.9                              & 74.3                              & 62.0                              \\
% MSMN                                       & 95.1                              & 95.5                              & 71.9                              & 75.8                              & 62.6                              \\
% \textbf{CoRelation}                        & \textbf{95.4}                     & \textbf{96.7}                     & \textbf{72.5}                     & \textbf{76.0}                     & \textbf{62.9}                     \\ \hline
% \textit{PLM-ICD}                                    & 95.0                              & 96.4                              & 71.4                              & 75.5                              & 62.4                              \\\hline
% \multicolumn{6}{c}{\textbf{MIMIC-IV-ICD10-50}}                                                                                                                                                                                 \\\hline
% CAML                                       & 91.1                              & 93.2                              & 64.3                              & 67.6                              & 59.6                              \\
% LAAT                                       & 93.2                              & 95.5                              & 68.2                              & 72.6                              & 64.4                              \\
% JointLAAT                                  & 93.4                              & 95.6                              & 68.4                              &  72.9                        & 64.5                              \\
% MSMN                                       & 93.6                              & 95.7                              & 70.3                              & 74.2                              & 65.2                              \\
% \textbf{CoRelation}                        & \textbf{93.8} & \textbf{96.0} & \textbf{70.6} & \textbf{74.4} & \textbf{65.4} \\ \hline
% \textit{PLM-ICD}                                    & 93.4                              & 95.6                              & 69.0                              & 73.3                              & 64.6                              \\\hline
% \end{tabular}
% \caption{Results on the MIMIC-IV-50 test sets.}
% \label{table:MIMIC-IV-50}
% \end{table}

\begin{table*}[h]
\centering
\caption{Results on the MIMIC-IV-50 test sets.}
\label{table:MIMIC-IV-50}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|ccccc|ccccc}
\hline
\multirow{3}{*}{Category}& \multirow{3}{*}{Method} &\multicolumn{5}{c|}{MIMIC-IV-\textbf{ICD9}-50}  & \multicolumn{5}{c}{MIMIC-IV-\textbf{ICD10}-50} \\ \cline{3-12}                                                                                                 
& & \multicolumn{2}{c}{AUC}                                               & \multicolumn{2}{c}{F1}                                                & Pre  & \multicolumn{2}{c}{AUC}                                               & \multicolumn{2}{c}{F1}                                                & Pre                              \\ \cline{3-12} 
    &                   & Macro                             & Micro                             & Macro                             & Micro                             & P@5   & Macro                             & Micro                             & Macro                             & Micro                             & P@5                             \\ \hline

PLM & {PLM-ICD}                                    & 95.0                              & 96.4                              & 71.4                              & 75.5                              & 62.4                              & 93.4                              & 95.6                              & 69.0                              & 73.3                              & 64.6                              \\\hline
\multirow{5}{*}{Non-PLM} 
& CAML                                       & 93.1                              & 94.1                              & 65.3                              & 69.2                              & 58.6   & 91.1                              & 93.2                              & 64.3                              & 67.6                              & 59.6                              \\
& LAAT                                       & 94.9                              & 96.3                              & 70.0                              & 74.5                              & 62.0                              & 93.2                              & 95.5                              & 68.2                              & 72.6                              & 64.4                              \\
& JointLAAT                                  & 94.9                              & 96.3                              & 69.9                              & 74.3                              & 62.0                              & 93.4                              & 95.6                              & 68.4                              &  72.9                        & 64.5                              \\
& MSMN                                       & 95.1                              & 95.5                              & 71.9                              & 75.8                              & 62.6                              & 93.6                              & 95.7                              & 70.3                              & 74.2                              & 65.2                              \\
\rowcolor{blue!25} 
\cellcolor{white}& {\model}                       & \textbf{95.4}                     & \textbf{96.7}                     & \textbf{72.5}                     & \textbf{76.0}                     & \textbf{62.9}                     & \textbf{93.8} & \textbf{96.0} & \textbf{70.6} & \textbf{74.4} & \textbf{65.4} \\ \hline

% \multicolumn{6}{c}{\textbf{MIMIC-IV-ICD10-50}}                                                                                                                                                                                 \\\hline
% CAML                                       & 91.1                              & 93.2                              & 64.3                              & 67.6                              & 59.6                              \\
% LAAT                                       & 93.2                              & 95.5                              & 68.2                              & 72.6                              & 64.4                              \\
% JointLAAT                                  & 93.4                              & 95.6                              & 68.4                              &  72.9                        & 64.5                              \\
% MSMN                                       & 93.6                              & 95.7                              & 70.3                              & 74.2                              & 65.2                              \\
% \textbf{CoRelation}                        & \textbf{93.8} & \textbf{96.0} & \textbf{70.6} & \textbf{74.4} & \textbf{65.4} \\ \hline
% \textit{PLM-ICD}                                    & 93.4                              & 95.6                              & 69.0                              & 73.3                              & 64.6                              \\\hline
\end{tabular}
}
\vspace{-0.2in}
\end{table*}

\subsection{Results of the 50 Setting}
In this section, we present the experimental outcomes for the three \textbf{50} settings, emphasizing the top 50 codes. In this setting, the size of $\mathcal{V}_d^\prime = 50$ for all data. A comprehensive comparison of methodologies on the MIMIC-III and MIMIC-IV settings is provided in Table~\ref{table:MIMIC-50} and Table~\ref{table:MIMIC-IV-50} respectively.
Results reveal that our proposed model, {\model}, outperforms all non-PLM methods across all metrics within the 50 settings. Even when compared to PLM methods, our method still demonstrates state-of-the-art performance on every metric, except for Micro F1 on the MIMIC-III-50 setting. Consequently, our method's advantage in the 50 settings is considerably substantial.



% \begin{table*}[ht]
% \centering
% \begin{tabular}{lccccccc}
% \hline
% \multicolumn{8}{c}{\textbf{MIMIC-III-Full}}                                                                                                                \\
% \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{AUC}       & \multicolumn{2}{c}{F1}        & \multicolumn{3}{c}{Pre}                       \\ \cline{2-8} 
% \multicolumn{1}{c}{}                       & Macro         & Micro         & Macro         & Micro         & P@5           & P@8           & P@15          \\ \hline
% CAML                                       & 89.5          & 98.6          & 8.8           & 53.9          & -             & 70.9          & 56.1          \\
% MultiResCNN                                & 91.0          & 98.6          & 8.5           & 55.2          & -             & 73.4          & 58.4          \\
% HyperCore                                  & 93.0          & 98.9          & 9.0           & 55.1          & -             & 72.2          & 57.9          \\
% LAAT                                       & 91.9          & 98.8          & 9.9           & 57.5          & 81.3          & 73.8          & 59.1          \\
% JointLAAT                                  & 92.1          & 98.8          & \textbf{10.7} & 57.5          & 80.6          & 73.5          & 59.0          \\
% TwoStage                                   & 94.6          & 99.0          & 10.5          & 58.4          & -             & 74.4          & -             \\
% MSMN                                       & 95.0          & \textbf{99.2} & 10.3          & 58.4          & 82.5          & 75.2          & 59.9          \\
% \textbf{CoRelation}                                 & \textbf{95.2} & \textbf{99.2} & 10.2          & \textbf{59.1} & \textbf{83.4} & \textbf{76.2} & \textbf{60.7} \\ \hline
% \textit{PLM-ICD}                                    & 92.5          & 98.9          & 8.4           & 58.0          & \underline{83.9}    & \underline{76.7}    & \underline{61.1}    \\ \hline
% \end{tabular}
% \caption{Results on the MIMIC-III-Full test set.}
% \label{table:MIMIC-FULL}
% \end{table*}
\begin{table}[ht]
\centering
\caption{Results on the MIMIC-III-Full test set.}
\label{table:MIMIC-FULL}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l|ccccccc}
\hline
% \multicolumn{8}{c}{\textbf{MIMIC-III-Full}}                                                                                                                \\
\multirow{2}{*}{Method} & \multicolumn{2}{c}{AUC}       & \multicolumn{2}{c}{F1}        & \multicolumn{3}{c}{Pre}                       \\ \cline{2-8} 
                      & Macro         & Micro         & Macro         & Micro         & P@5           & P@8           & P@15          \\ \hline
{PLM-ICD}                                    & 92.5          & 98.9          & 8.4           & 58.0          & \underline{83.9}    & \underline{76.7}    & \underline{61.1}    \\ \hline
CAML                                       & 89.5          & 98.6          & 8.8           & 53.9          & -             & 70.9          & 56.1          \\
MultiResCNN                                & 91.0          & 98.6          & 8.5           & 55.2          & -             & 73.4          & 58.4          \\
HyperCore                                  & 93.0          & 98.9          & 9.0           & 55.1          & -             & 72.2          & 57.9          \\
LAAT                                       & 91.9          & 98.8          & 9.9           & 57.5          & 81.3          & 73.8          & 59.1          \\
JointLAAT                                  & 92.1          & 98.8          & \textbf{10.7} & 57.5          & 80.6          & 73.5          & 59.0          \\
TwoStage                                   & 94.6          & 99.0          & 10.5          & 58.4          & -             & 74.4          & -             \\
MSMN                                       & 95.0          & \textbf{99.2} & 10.3          & 58.4          & 82.5          & 75.2          & 59.9          \\
\rowcolor{blue!25} 
{\model}                                & \textbf{95.2} & \textbf{99.2} & 10.2          & \textbf{59.1} & \textbf{83.4} & \textbf{76.2} & \textbf{60.7} \\ \hline
\end{tabular}
}
\end{table}


\begin{table*}[h]
\centering
\caption{Results on the MIMIC-IV-Full test sets.}
\label{table:MIMIC-IV-FULL}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|ccccc|ccccc}
\hline
\multirow{3}{*}{Category}& \multirow{3}{*}{Method} &\multicolumn{5}{c|}{MIMIC-IV-\textbf{ICD9}-Full}  & \multicolumn{5}{c}{MIMIC-IV-\textbf{ICD10}-Full} \\ \cline{3-12}                                                                                                 
& & \multicolumn{2}{c}{AUC}                                               & \multicolumn{2}{c}{F1}                                                & Pre  & \multicolumn{2}{c}{AUC}                                               & \multicolumn{2}{c}{F1}                                                & Pre                              \\ \cline{3-12} 
    &                   & Macro                             & Micro                             & Macro                             & Micro                             & P@8   & Macro                             & Micro                             & Macro                             & Micro                             & P@8                             \\ \hline

PLM & {PLM-ICD}                                   & 96.6       & 99.5       & 14.4       & \underline{62.5}      & \underline{70.3}        & 91.9      & 99.0      & 4.9       & 57.0     & 69.5                              \\\hline
\multirow{5}{*}{Non-PLM} 
& CAML                                       & 93.5       & 99.3       & 11.1       & 57.3      & 64.9        & 89.9      & 98.8      & 4.1       & 52.7     & 64.4\\
& LAAT                                      & 95.2       & 99.5       & 13.1       & 60.3      & 67.5              & 93.0      & 99.1      & 4.5       & 55.4     & 67.0  \\
& JointLAAT                                  & 95.6       & 99.5       & 14.2       & 60.4      & 67.5     & 93.6      & 99.3      & 5.7       & 55.9     & 66.9 \\
& MSMN                                       & \textbf{96.8}       &  \textbf{99.6}       & 13.9       & 61.2      & 68.9     & 97.1      & \textbf{99.6}      & 5.4       & 55.9     & 67.7  \\
\rowcolor{blue!25} 
\cellcolor{white}& {\model}                  & \textbf{96.8}       &  99.5       & \textbf{15.0}       & \textbf{62.4}      & \textbf{70.1}      &\textbf{97.2}       & \textbf{99.6}       & \textbf{6.3}        & \textbf{57.8}      & \textbf{70.0}\\ \hline

% \multicolumn{6}{c}{\textbf{MIMIC-IV-ICD10-50}}                                                                                                                                                                                 \\\hline
% CAML                                       & 91.1                              & 93.2                              & 64.3                              & 67.6                              & 59.6                              \\
% LAAT                                       & 93.2                              & 95.5                              & 68.2                              & 72.6                              & 64.4                              \\
% JointLAAT                                  & 93.4                              & 95.6                              & 68.4                              &  72.9                        & 64.5                              \\
% MSMN                                       & 93.6                              & 95.7                              & 70.3                              & 74.2                              & 65.2                              \\
% \textbf{CoRelation}                        & \textbf{93.8} & \textbf{96.0} & \textbf{70.6} & \textbf{74.4} & \textbf{65.4} \\ \hline
% \textit{PLM-ICD}                                    & 93.4                              & 95.6                              & 69.0                              & 73.3                              & 64.6                              \\\hline
\end{tabular}
}
\end{table*}

\subsection{Results of the Full Setting}
Next, we examine the results of three \textbf{Full} settings in Table~\ref{table:MIMIC-FULL} and Table~\ref{table:MIMIC-IV-FULL}.
For the Full settings, only one PLM method is included since other PLM methods cannot handle the huge potential label space as illustrated in Table~\ref{table:datasets}.
{\model} once again outperforms existing non-PLM methods across a majority of metrics within the MIMIC-III-Full, MIMIC-IV-ICD9-Full, and MIMIC-IV-ICD10-Full contexts. 
%These findings suggest our proposed model's effectiveness and advancement under the Full code settings. 
Concurrently, it is important to note that the improvement of {\model} in Precision at $\mathcal{K}$ (P@$\mathcal{K}$) scores is particularly significant, demonstrating that the proposed relation learning technique is effective in refining high-probability code predictions.
Compared to PLM methods, although PLM-ICD exhibits superior performance in some P@$\mathcal{K}$ metrics, its underwhelming performance across other metrics - including its poor results in the 50 settings - renders it less competitive. Besides, our model operates with considerably fewer parameters (22 Million vs. 120 Million) compared to PLM methods. As such, the advantage of the {\model} remains evident.


\subsection{Ablation Study}
In this section, we present an ablation study to examine the contribution of each proposed module to the overall performance of our model. The results are summarized in Table~\ref{table:ABA}. The following notations represent different configurations of our model:

\begin{itemize}
\item \textbf{W/O Relation}: This notation signifies our proposed model without the application of the relation learning discussed in Section~\ref{section:code2code}.

\item \textbf{W/O Flexible Relation Graph (W/O FRG)}: This is the configuration where our proposed flexible relation graph, described in Section~\ref{section:flex}, is replaced with a fixed ICD ontology + co-occurrence graph, similar to~\cite{cao2020hypercore}.

\item \textbf{W/O Context}: This denotes a version of our model that excludes the use of contextualized code embeddings, as per Section~\ref{sec:cont}. The non-contextualized code description embeddings $\mathbf{s}_{i,j}$ are employed to initialize the relation graph $\mathcal{G}_d^\prime$, similar to~\cite{xie2019ehr, cao2020hypercore}.

\item \textbf{W/O Self-Adaptive Aggregation (W/O SAA)}: This indicates our proposed model without the integration of the self-adaptive aggregation discussed in Section~\ref{sec:agg}. The $\mathbf{P}_g$ is directly employed as the final output.
\end{itemize}

We initiate the comparison with \textbf{W/O Relation} and the proposed model. Under both the 50 and Full settings, the omission of the relation results in a decline in most metrics, signifying the efficacy of our proposed relation learning in managing both frequent code settings and full code settings. Concurrently, we individually substitute components of the proposed contextualized relation learning to evaluate the efficiency of each proposed module. \textbf{W/O FRG} incurs the smallest decrease, yet it does not suggest that the contribution of flexible relation modeling is trivial. As the flexible relation graph centers on intricate and weak relationships, its enhancements are less apparent in quantitative analysis. The case studies in Section~\ref{sec:case} will illustrate that the relations inferred within the flexible graph hold significant value.
Finally, both \textbf{W/O SAA} and \textbf{W/O Context} contribute to substantial declines in the final performance. This underlines the significance of contextualized relation modeling and self-adaptive aggregation. 
%Without the inclusion of these two proposed methods, merely introducing the relation information would result in the model learning detrimental features. 
In conclusion, all the proposed module contribute to the ultimate performance.
\begin{table*}[h]
\vspace{-0.2in}
\centering
% \vspace{-0.15in}
\caption{Results of ablation experiments on the MIMIC-III datasets.}
\label{table:ABA}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ccccccc|ccccccc}
\hline
Dataset & \multicolumn{6}{|c|}{MIMIC-III-50}                                                                                                                                                                                                                     & \multicolumn{6}{c}{MIMIC-III-Full}                                                                                                                                                                  \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Method}}   & \multicolumn{2}{c}{AUC}                                         & \multicolumn{2}{c}{F1}                                          & \multicolumn{2}{c|}{Pre}                                         & \multicolumn{2}{c}{AUC}                                         & \multicolumn{2}{c}{F1}                                          & \multicolumn{3}{c}{Pre}                                         \\\cline{2-14}
\multicolumn{1}{c|}{}                          & Macro                          & Micro                          & Macro                          & Micro                          & P@5                            & P@8                            & Macro                          & Micro                          & Macro                          & Micro                          & P@5                            & P@8      & P@15                       \\ \hline
\rowcolor{blue!25}
\multicolumn{1}{l|}{\model} & \textbf{93.3} & \textbf{95.1} & \textbf{69.3} & \textbf{73.1} & \textbf{68.3} & \textbf{55.6} & \textbf{95.2} & \textbf{99.2} & 10.2  & \textbf{59.1} & \textbf{83.4} & \textbf{76.2} & \textbf{60.7}\\
\multicolumn{1}{l|}{W/O Relation}              & 93.1                           & 95.0                           & 69.0                           & 72.6                           & 68.1                           & 55.2                           & 95.2                           & 99.1                           & 9.3                            & 58.9                           & 82.8                           & 75.7     & 60.5                      \\ \hline
\multicolumn{1}{l|}{W/O FRG}              & 93.2                           & 95.1                           & 69.0                           & 72.9                           & 68.2                           & 55.5                           & 95.1                           & 99.2                           & 10.0                           & 58.8                           & 83.3                           & 76.0             & 60.5              \\
\multicolumn{1}{l|}{W/O Context}               & 92.0                           & 93.7                           & 66.4                           & 70.0                           & 66.2                           & 53.8                           & 95.0                           & 99.1                           & \textbf{10.7} & 57.9                           & 81.4                           & 74.3               & 59.4            \\
\multicolumn{1}{l|}{W/O SAA}              & 92.5                           & 94.7                           & 68.6                           & 72.2                           & 67.9                           & 55.0                           & 95.0                           & 99.1                           & 9.7                            & 58.8                           & 82.9                           & 75.9        & 60.1                   \\ \hline
\end{tabular}
}
\vspace{-0.15in}
\end{table*}

\subsection{Case Study on Learned Code Relations}\label{sec:case}
To better comprehend the efficacy of our proposed flexible, context-aware code relationship learning in facilitating code prediction, we conduct case studies to elucidate the relationships inferred from the code. The cases are depicted in Figure~\ref{fig:case}. Based on our analysis, the inferred relationships can be categorized into two types.

\textbf{Type 1} relationships concentrate on differentiating similar codes by referencing codes that originate from the same family. For example, the top-3 referenced codes for the code ``584.9'' (\textit{Acute kidney failure}) are ``586'' (\textit{Renal failure}), ``580'' (\textit{Acute glomerulonephritis}), and ``582'' (\textit{Chronic glomerulonephritis}). All these referenced codes, including ``584.9'', are part of the \textit{Kidney disorder family}. The model, by taking these analogous codes into consideration, can make more precise predictions by discerning subtle differences.


\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/cases.pdf}
\caption{Two typical learned code relation cases.}
\vspace{-0.2in}
\label{fig:case}
\end{figure}

\textbf{Type 2} relationships focus on referencing codes that demonstrate specific associations. For instance, the top-3 cited codes for ``788.20'' (\textit{Urinary retention}) are ``280'' (\textit{Iron deficiency anemias}), ``286'' (\textit{Other unspecified anemias}), and ``281'' (\textit{Hereditary hemolytic anemias}), all falling under the \textit{Anemia} category. The incidence of \textit{Urinary Retention} is frequently associated with the severity of \textit{anemia}~\cite{hung2015association}. By utilizing flexible relationship learning, the model is capable of recognizing such associations and employing them to bolster prediction outcomes.

To summarize, the relationships inferred within the flexible graph are highly interpretable and exhibit a robust correlation with real-world medical practices.



\subsection{Evaluation of Top-$K$ Code Selection}


\begin{table}[t]
\centering
\footnotesize
\caption{Evaluation of $K$ values on the MIMIC-III-Full.}
\label{table:k}
\begin{tabular}{l|cc|cc|c}
\hline
\multirow{2}{*}{$K$} & \multicolumn{2}{c|}{AUC} & \multicolumn{2}{c|}{Pre} & \multirow{2}{*}{Memory} \\ \cline{2-5}
                           & Macro       & Micro      & P@5        & P@8        &                         \\ \hline
$300$                    &  95.2     &  99.2    & 83.4       & 76.2       & 9.15 GB                 \\
$200$                    &  95.2     &  99.2    & 83.5       & 76.1       & 7.78 GB                 \\
$100$                    &  95.2     &  99.2    & 83.1       & 75.8       & 6.41 GB                 \\
$50$                     &  95.1     &  99.2    & 83.0       & 75.4       & 5.05 GB                 \\ \hline
\end{tabular}
\vspace{-0.25in}
\end{table}
In this section, we evaluate the efficacy of the top-$K$ code selection strategy, delineated in Section~\ref{section:flex}. We manipulate $K$ within a range of 50 to 300, and the corresponding performance metrics along with per-sample GPU memory costs are compiled in Table~\ref{table:k}. It is clear that escalating values of $K$ bolster the performance of our model, albeit at the cost of increased GPU memory consumption. Nevertheless, the marginal performance enhancement decelerates as $K$ keeps surging, predominantly due to the dwindling influence of the remaining low-probability codes, elucidated in Section~\ref{section:flex}. This indicates that our proposed top-$K$ code selection strategy is potent, without compromising the overall model performance.



\subsection{Evaluation of Major Code Substitution}
\begin{table}[t]
\centering
\footnotesize
\caption{Evaluation of Major Code Substitution on the MIMIC-III-50 dataset.}
\label{table:major}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|cc|c|c|c}
\hline
\multirow{2}{*}{Method}       & \multicolumn{2}{c|}{AUC} & \multirow{2}{*}{P@5} & \multirow{2}{*}{Memory} & \multirow{2}{*}{Time} \\ \cline{2-3}
                                & Macro      & Micro      &                      &                         &                       \\ \hline
\multicolumn{1}{c|}{Complete}  & 93.3       & 95.1       & 68.4                 & 6.0 GB                  & 0.23s                  \\
\multicolumn{1}{c|}{Major} & 93.3       & 95.1       & 68.3                 & 1.5 GB                  & 0.05s                 \\ \hline
\end{tabular}}

\end{table}
We also assess the efficacy of the proposed major code substitution strategy in Section~\ref{section:flex}, and the results are shown in Table~\ref{table:major} on the MIMIC-III-50 dataset. 
The term \textbf{Complete} indicates the strategy where the upper-level codes, denoted as $\mathcal{U}$, are not replaced with the major codes $\mathcal{U}^\prime$. Conversely, \textbf{Major} refers to the implementation of the major code substitution strategy. The reported speed and memory costs are the average per-sample metrics observed during training.
As can be deduced from Table~\ref{table:major}, employing the major code substitution results in a substantial decrease in memory usage and computational time while sustaining a performance level comparable to the complete approach.

\subsection{Evaluation of the Selective Training}
\begin{table}[t]
\vspace{-0.15in}
\centering
\caption{GPU memory space comparison results on the MIMIC-III-Full setting.}
\label{table:Eff}
\begin{tabular}{c|cc}
\hline
     Method                                                        & Memory  \\ \hline
{\model} Selective & 9.15 GB                   \\
{\model} W/O Selective                                                       & 72.76GB                  \\ \hline
%PLM-ICD                                                       & 19.29GB               \\\hline
\end{tabular}
\vspace{-0.15in}
\end{table}
To prove the efficiency of the proposed selective training method, we report the per-sample space cost results in Table~\ref{table:Eff}.
From Table~\ref{table:Eff}, we can discover that our proposed selective training approach significantly reduces memory cost. By utilizing a more efficient training strategy that selectively samples the code space, our method drastically reduces GPU memory usage from 72.76 GB to just 9.15 GB by nearly 12.5\% of the original cost.




==> files/method_new.tex <==
\section{Methodology}
\subsection{Contextualized Code Embedding Extraction}
Inspired by recent work MSNM~\cite{yuan2022code}, we propose a synonym-based code encoding framework with standard key-query attention to directly obtain relevant features from clinical notes by referring to the ICD code description at the initial stage. Specifically, we employ the same text encoder to encode both the raw clinical note and the code descriptions. Here, each $c_i\in\mathcal{C}$ contains $s$ synonym descriptions of code $c_i$.
\begin{align}
    \mathbf{H} = \text{TextEncoder}(\mathcal{D})\label{eq:textencoder}\\
    \mathbf{C} = \text{TextEncoder}(\mathcal{C})
\end{align}
Let $\mathbf{H}$ be the encoded dense representation of the note $\mathcal{D}$, and $\mathbf{C}$ be the encoded representation of the codes $\mathcal{C}$, where $\mathbf{H}\in \mathbb{R}^{l\times e}$ and $\mathbf{C}\in \mathbb{R}^{p\times s\times e}$. The dimension $e$ represents the embedding dimension.

Next, we utilize a standard key-query attention layer~\cite{vaswani2017attention} to extract code-related features from the text embedding $\mathbf{H}$:
\begin{equation}
\mathbf{E}_{c}^{multi} = \text{KeyQueryAttention}(\mathbf{C}, \mathbf{H})
\label{eq:keyquery}
\end{equation}
Here, $\mathbf{E}_{c}^{multi}\in \mathbb{R}^{p\times s \times e}$ represents the obtained multi-synonymy representations. For each code, we use maximum pooling to obtain an overall representation across the synonym dimension $s$:
\begin{equation}
\mathbf{E}_{c} = \text{MaxPool}(\mathbf{E}_{c}^{multi})
\label{eq:maxpool}
\end{equation}
In the meanwhile we also extract the major code embeddings $\mathbf{E}_{mc}$ using a similar approach. Here, major codes refer to the parent codes of each leaf-level ICD code. For example, the major code of "214.2 (Lipoma of intrathoracic organs)" is "214 (Lipoma)". Those major code embeddings will be used to replace the general codes to improve efficiency, which we are going to describe in Section~\ref{sec:sub}.
Likewise, we employ the MSyn module (Eqs~\eqref{eq:textencoder}-\eqref{eq:maxpool}) to extract features related to major codes from the clinical note $\mathcal{D}$, leveraging the information provided by the simplified major code group $\mathcal{C}_{mc}$.
\begin{equation}
    \mathbf{E}_{mc} = \text{MSyn}(\mathcal{C}_{mc}, \mathcal{D})
\end{equation}
Subsequently, we apply a fully connected layer to obtain the prediction matrix $\mathbf{W}_{c}\in \mathbb{R}^{p \times e}$ of the code embedding matrix $\mathbf{C}$. In order to encourage the model to generate similar embeddings for different synonym representations, we employ the average operation to obtain the final prediction matrix by averaging the representations from the synonym embeddings before sending the fully connected (FC) transform layer:
\begin{equation}
\mathbf{W}_{c} = \text{FC}_c(\text{Average}(\mathbf{C}))
\end{equation}
Finally, the direct inference probability is calculated by taking the inner product of the prediction matrix and the extracted code-related features, followed by applying the sigmoid activation function $\sigma()$:
\begin{equation}
\mathbf{P}_{c} = \sigma(\mathbf{W}_{c}\cdot\mathbf{E}_{c})
\end{equation}
This result stands for the initial direct prediction result, and we are going to use code-to-code relation learning to improve it further.
\subsection{Gated Code-to-code Relation Learning}\label{section:code2code}
In addition to direct prediction results, experts frequently rely on code-to-code relations during the ICD coding process to polish the previous assigned ICD codes. These relations offer valuable context and emphasize connections between relevant codes, aiding in more accurate code assignment.

To enhance and streamline the ICD coding process, we propose a novel prediction network called the gated code-to-code relation learning module. This network aims to capture the intricate relationships between ICD codes, ultimately improving the accuracy of code assignment.  However, directly modeling the relations on the original ICD tree graph is complicated due to its hierarchical structure with multiple layers. As illustrated in Figure~\ref{fig:bipartite} (a), if $c_1$ wants to exchange information with $c_2$, four rounds of information passing are required. Consequently, previous approaches~\cite{xie2019ehr, cao2020hypercore} can only model the relationships offline during the prepossessing stage without involving the contexts.
To address this issue, we employ a simplified bipartite graph to represent the code-to-code connections, as depicted in Figure~\ref{fig:bipartite} (b). This allows each code to communicate with all the codes in a single round.
\begin{figure}[h]
\centering
\includegraphics[width=0.8\linewidth]{images/bipartial.pdf}
\caption{We simplify the original hierarchical ICD tree graph into a directed bipartite graph. There is an edge for each code pair code, and the type of the edge is dependent by the distance between two codes on the original ICD tree.}
\label{fig:bipartite}
\end{figure}
\subsubsection{Major Code Substitution Strategy}\label{sec:sub}
\begin{figure}[h]
\centering
\includegraphics[width=0.4\linewidth]{images/sub.pdf}
\caption{Substituted bipartite graph.}
\label{fig:sub}
\end{figure}
However, the computational cost is substantial. In the full setting, there are a total of $8,921\times 8,921$ edges. To further reduce the computational burden, we replace the upper part codes with the major codes as shown in Figure~\ref{fig:sub}, which only amounts to 1,158 cases. The lower-level codes are used to predict the final results; thus, we only replace the upper part. 
Since ICD codes belonging to the same major code generally do not coexist in the same case, this substitution does not significantly impact performance.
\subsubsection{Relation Modeling}
Then, we use graph transformer~\cite{dwivedi2020generalization} to model the interaction between codes. 
\begin{equation}
    \mathbf{E}_{c}^{mc} = \text{GraphTransformer}(\mathbf{E}_{c}, \mathbf{E}_{mc},\mathbf{E}_{r})
\end{equation}
Here, $\mathbf{E}_{r}\in \mathbb{R}^{p \times p_{mc} \times e_r}$ represents the embeddings of relation types in the bipartite graph, where $p_{mc}$ is the number of major codes, and $e_r$ is the dimension of each relation embedding. The features of the codes, $\mathbf{E}_{c}$, and $\mathbf{E}_{mc}$, are extracted from the input clinical note, $\mathcal{D}$, in real-time, which are sued to represent the lower-level and upper-level parts contextualized code embeddings.
Therefore, our approach to modeling relationships between codes is dynamic and context-aware, boasting impressive flexibility. This approach diverges from prior techniques~\cite{xie2019ehr, cao2020hypercore}, which used preprocessing procedures to model a static code relationship graph.
The resulting enhanced embeddings $\mathbf{E}_{c}^{mc} \in \mathbb{R}^{p \times e}$ from the lower-level codes are then used to estimate a new probability $\mathbf{P}_{mc}$:
\begin{align}
    \mathbf{P}_{mc} &= \sigma(\mathbf{W}_{mc}\mathbf{E}_c^{mc})\\
    \mathbf{W}_{mc} &= \text{Average}(\mbox{FC}_{mc}(\mathbf{C})))
\end{align}
\subsection{Self-adaptive Gate}
We then use the raw activation result (element-wise product $\odot$ of $\mathbf{W}_{c}$ and $\mathbf{E}_{c}$) from the MSyn module to calculate the proportion value $\mathbf{A}_{c}^{mc}$ of code-to-code inference, which can make model pay more attention to the complex code-to-code inference only when it is necessary to avoid the abusing of code-to-code inference results. 
\begin{align}
    \mathbf{A}_{mc} &= \sigma(\mbox{FC}_{a}(\mathbf{W}_{c}\odot\mathbf{E}_{c}))
\end{align}
The final prediction result $\mathbf{P}$ is the gated combination of two prediction results.
\begin{align}
\mathbf{P} = &(1-\mathbf{A}_{mc} )\odot\mathbf{P}_{c}+\mathbf{A}_{mc}\odot\mathbf{P}_{mc}\label{eq:gate}
\end{align}
The training loss for the final prediction results is:
\begin{equation}
     \mathcal{L}_{CE} = \text{CrossEntropy}(\mathbf{P}, \mathbf{G})
\end{equation}
$\mathbf{G}$ is the ground-truth label.
In the meanwhile, we use the following loss to encourage the model to use less complex features by making the average proportion value $\mathbf{A}_{mc}$ as a loss term.
\begin{equation}
     \mathcal{L}_{comp} = \text{Average}(\mathbf{A}_{mc})
\end{equation}
The final training loss is:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{CE}+\beta\mathcal{L}_{comp}
\end{equation}
Where, $\beta$ is the hyper-parameters for controlling the importance of ${L}_{comp}$.
\subsection{Sampling Training Strategy}\label{sec:sampling}
In ICD coding, the majority of codes possess a limited number of positive labels. The average positive labels for each case under the MIMIC-III-full setting is 15. However, there are total of 8,921 labels. Consequently, for full settings, most prediction results consist of negative labels. Despite contributing minimal gradients for model updates, these negative labels still demand equal computational resources during backpropagation. To circumvent this computational inefficiency, we propose a sampling-based training algorithm, detailed in Algorithm~\ref{alg:cap}.
\begin{algorithm}[h]
\footnotesize
\caption{Sampling Training}\label{alg:cap}
\KwIn{Code set $\mathcal{C}$, dataset $\mathbb{D}$, and model parameter $\theta$.}
\KwOut{Updated model parameter $\theta$.}
\While{Training not finished}{
1. Sampling $\mathcal{D}, \mathbf{G}$ from data set $\mathbb{D}$ \\
$\mathcal{D}, \mathbf{G}\gets\mathbb{D}$ \\
2. Perform forward propagation without code relation to estimate the scores.\\
$\hat{\mathbf{P}_{est}} = {\text{\model}}_{wo}(\mathcal{C}, \mathcal{D})$\\
3. Choose top $k_1$ codes for ${\text{\model}}_{wo}$ prediction training.\\
$\mathcal{C}_{top k_1}=\{\cdots, c_i, \cdots\}, i \in \text{TopK}(\hat{\mathbf{P}_{est}}, k_1)$\\
4. Choose top $k_2$ codes for $\text{\model}$ prediction training.\\
$\mathcal{C}_{top k_2}=\{\cdots, c_i, \cdots\}, i \in \text{TopK}(\hat{\mathbf{P}_{est}}, k_2)$\\
5. Adding additional $k_1$ random codes, the ground-truth codes, and removing the training codes for $\text{\model}$ to form $\mathcal{C}_{1}$.\\
$\mathcal{C}_{1}=\{\mathcal{C}_{top k_1},\mathcal{C}_{ground}, \mathcal{C}_{random}\}-\mathcal{C}_{top k_2}$\\
6. Perform forward calculation for the selected codes only.\\
$\mathbf{P}_{1}= {\text{\model}}_{wo}(\mathcal{C}_{1}, \mathcal{D})$\\
$\mathbf{P}_{2}= \text{\model}(\mathcal{C}_{topk_2}, \mathcal{C}_{mc}, \mathcal{D})$\\
$\mathbf{P}= \mathbf{P}_{1}\oplus\mathbf{P}_{2}$\\
7. Calculate the loss $\mathcal{L}$.\\
$\mathcal{L} = LossFunc(\mathbf{P}, \mathbf{G})$\\
8. Update model parameter $\theta$.\\
$\theta = \theta- \nabla L$\\
}
\end{algorithm}

Specifically, we initially choose the top $k_1, k_2$ training codes for $\text{\model}_{wo}$ and $\text{\model}$ (steps 1-5), then only perform backpropagation on these chosen codes (steps 6-8). Here, $\text{\model}_{wo}$ means directly predicting the results without using code-to-code relation learning in Section~\ref{section:code2code}. $k_2$ is smaller than $k_1$ since $\text{\model}$ requires more computation resource than $\text{\model}_{wo}$.
This sampling-based training algorithm enables the model to focus on the most relevant codes during training, thereby reducing computational resources and avoiding the expenditure on negative labels that provide minimal gradient information.

%\subsection{Training Loss}
%To make the model learn more robust features, we follow the previous work MSMN~\cite{yuan2022code} to add the R-Drop~\cite{wu2021r} loss to regularize the learned feature.
%\begin{equation}
%\begin{split}
%    \mathcal{L}_{drop} = \frac{1}{2}(\mathcal{D}_{KL}(\sigma(logit_1)||(\sigma(logit_2))\\+\mathcal{D}_{KL}(\sigma(logit_2)||(\sigma(logit_1)))
%\end{split}
%\end{equation}
%Where $logit_1$ and $logit_2$ are output logits of the model with two different random drop for the same input.
%The final training loss is:
%\begin{equation}
%    \mathcal{L} = \mathcal{L}_{CE}+\beta\mathcal{L}_{comp}
%\end{equation}
%Where, $\beta$ is the hyper-parameters for controlling the importance of ${L}_{comp}$.

==> files/old.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|lccccccc}
\hline
\multirow{2}{*}{MIMIC-III-full}                                   & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{AUC}                                         & \multicolumn{2}{c}{F1}                                             & \multirow{2}{*}{P@5}           & \multirow{2}{*}{P@8}  & \multirow{2}{*}{P@15}          \\
                                 & \multicolumn{1}{c}{}                              & Macro                          & Micro                          & Macro                          & Micro                             &                                &                                \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Non-PLM\\ Methods\end{tabular}}&CAML        & 89.5            & 98.6  & 8.8   & 53.9     &   -   & 70.9                 & 56.1                                      \\
%MSATT-KG    & 91.0            & 99.2  & 9.0   & 55.3     &      & 72.8                 & 58.1                                      \\
&MultiResCNN & 91.0            & 98.6  & 8.5   & 55.2     &  -    & 73.4                 & 58.4                                      \\
&HyperCore   & 93.0            & 98.9  & 9.0   & 55.1     &  -    & 72.2                 & 57.9                                      \\
&LAAT        & 91.9            & 98.8  & 9.9  & 57.5     &  81.3    & 73.8                 & 59.1                                      \\
&JointLAAT   & 92.1            & 98.8  & \textbf{10.7}  & 57.5     & 80.6     & 73.5                 & 59.0                                      \\
&TwoStage        & 94.6            & 99.0  & 10.5  & 58.4     &  -    & 74.4                 & -                                      \\
&MSMN        & 95.0            & \textbf{99.2}  & 10.3  & 58.4     &  82.5    & 75.2                 & 59.9                                      \\
%KEPT        & -               & -     & -     & -        &  -    & -                    & -                                         \\  \hline
&\textbf{\model}     & \textbf{95.2}   & \textbf{99.2}  & 10.2   & \textbf{59.1} & \textbf{83.4} & \textbf{76.2}        & \textbf{60.7}                             \\ \hline
%&$\text{\model}_{base}$        & 94.4            & 99.0  & 9.8  & 57.8     &  82.5    & 75.0                 & 59.5                                      \\
\multirow{1}{*}{PLM Methods}&\textit{PLM-ICD}        & 92.4            & 98.9  & 8.4  & 57.8     &  \underline{83.7}    & \underline{76.5}                 & \underline{60.8}                                      \\ \hline
%ERI         & 2.0\%                &       &       &       & 5.7\%         &  1.6\%               & 1.2\%                                     \\ \hline
\end{tabular}
\caption{Results on the MIMIC-III-Full test set.}
\label{table:MIMIC-FULL}
\end{table*}
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{l|ccccc}
\hline
 \multirow{2}{*}{full}   & \multirow{2}{*}{P@5} & \multirow{2}{*}{P@8} & \multirow{2}{*}{P@15}  & \multirow{2}{*}{Memory}\\
                                &                      &                      &                       \\ \hline
                                %$k=300$                   & 95.2       & 99.2       & 10.2        & 59.1      & 83.4                 & 76.2                 & 60.7                  \\
                                %$k=200$                   & 95.2       & 99.2       & 9.9         & 59.0      & 83.5                 & 76.1                 & 60.7                  \\ 
                                %$k=100$                   & 95.1       & 99.2       & 10.0        & 58.9      & 83.1                 & 75.8                 & 60.5                  \\ 
                                %$k=50$                    & 95.1       & 99.2       & 10.0        & 58.9      & 83.0                 & 75.4                 & 60.4                  \\ \hline
                                $k=300$                        & 83.4                & 76.2                 & 60.7 & 9.15 GB                 \\
                                $k=200$                                & 83.5                 & 76.1                 & 60.7 & 7.78 GB                  \\ 
                                $k=100$                             & 83.1                 & 75.8                 & 60.5   & 6.41 GB                \\ 
                                $k=50$                              & 83.0                 & 75.4                 & 60.4  & 5.05 GB                 \\ \hline
\end{tabular}
\caption{Evaluation of $k$ value on MIMIC-III-Full.}
\label{table:k}
\end{table}

\begin{table*}[h]
\centering
\footnotesize
\caption{Ablation experiment results.}
\label{table:ABA}
\begin{tabular}{c|c|ccccccc}
\hline
\multirow{2}{*}{Dataset}        & \multirow{2}{*}{Method} & \multicolumn{2}{c}{AUC} & \multicolumn{2}{c}{F1} & \multicolumn{3}{c}{Pre}  \\
                                &                         & Macro      & Micro      & Macro      & Micro     &  P@5                    &  P@8                    &  P@15                     \\ \hline
\multirow{5}{*}{MIMIC-III-50}   & {\model}           & \textbf{93.3}       & \textbf{95.1}       & \textbf{69.3}      & \textbf{73.1}      & \textbf{68.3}                 & \textbf{55.6}                 & -                     \\
                                & W/O Relation                    & 93.1       & 95.0       & 69.2      & 72.6      & 68.1                 & 55.2                 & -                     \\\cline{2-9}
                                & W/O Flexible               & 93.2       & 95.1       & 69.0       & 72.9      & 68.2                 & 55.5                 & -                     \\ 
                                & W/O Adaptive                & 92.5       & 94.7       & 68.6       & 72.2      & 67.9                 & 55.0                 & -                     \\ 
                                & W/O Context               & 92.0       & 93.7       & 66.4       & 70.0      & 66.2                 & 53.8                 & -                     \\\hline
\multirow{5}{*}{MIMIC-III-Full} & {\model}           & \textbf{95.2}       & \textbf{99.2}       & 10.2       & \textbf{59.1}      & \textbf{83.4}                 & \textbf{76.2}                 & \textbf{60.7}                  \\
                                & W/O Relation                    & 95.2       & 99.1       & 9.3        & 58.9      & 82.8                 & 75.7                 & 60.5                  \\\cline{2-9} 
                                 & W/O Flexible               & 95.1       & 99.2       & 10.0       & 58.8      & 83.3                 & 76.0                 & 60.5                     \\
                                & W/O Adaptive                    & 95.0       & 99.1       & 9.7        & 58.8      & 82.9                 & 75.9                 & 60.1                  \\
                                & W/O Context               & 95.0       & 99.1       & \textbf{10.7}       & 57.9      & 81.4                 & 74.3                 & 59.4                     \\\hline
\end{tabular}
\end{table*}
